SafePowerGraph-HIL: Real-Time HIL Validation of Heterogeneous GNNs for Bridging Sim-to-Real Gap in Power Grids

As machine learning (ML) techniques gain prominence in power system research, validating these methods' effectiveness under real-world conditions requires real-time hardware-in-the-loop (HIL) simulations. HIL simulation platforms enable the integration of computational models with physical devices, allowing rigorous testing across diverse scenarios critical to system resilience and reliability. In this study, we develop a SafePowerGraph-HIL framework that utilizes HIL simulations on the IEEE 9-bus system, modeled in Hypersim, to generate high-fidelity data, which is then transmitted in real-time via SCADA to an AWS cloud database before being input into a Heterogeneous Graph Neural Network (HGNN) model designed for power system state estimation and dynamic analysis. By leveraging Hypersim's capabilities, we simulate complex grid interactions, providing a robust dataset that captures critical parameters for HGNN training. The trained HGNN is subsequently validated using newly generated data under varied system conditions, demonstrating accuracy and robustness in predicting power system states. The results underscore the potential of integrating HIL with advanced neural network architectures to enhance the real-time operational capabilities of power systems. This approach represents a significant advancement toward the development of intelligent, adaptive control strategies that support the robustness and resilience of evolving power grids.

==> pages/2-problem_formulation.tex <==
The AC-OPF problem is formulated as follows:
\begin{align}
\min_{p, q, v} \quad & \sum_{i=1}^{N} c_i(p_i) \\
\text{s.t.} \quad & p + jq = \text{diag}(v)(Xv)^*, \\
& V_{\min} \leq |v| \leq V_{\max}, \\
& p_{\min} \leq p \leq p_{max}, \quad q_{min} \leq q \leq q_{max}, \\
& s_{ij}(v) \leq \bar{s}_{ij}, \quad \forall (i, j) \in \mathcal{E}.
\vspace{-0.5em}
\end{align}
Where:
\begin{itemize}
\item \( p \) and \( q \) are the vectors of active and reactive power injections at each node, respectively.
\item \( c_i(p_i) \) represents a cost curve that is monotonically increasing and convex.
\item \(X\) is the given network admittance matrix (X-bus).
\item \( v \) is the vector of complex nodal voltages.
\item \( V_{\min} \) and \( V_{\max} \) are the specified lower and upper voltage magnitude limits, respectively.
\item \( p_{\min} \), \( p_{\max} \), \( q_{\min} \), and \( q_{\max} \) are the lower and upper bounds for active and reactive power injections.
\item \( s_{ij}(v) \) denotes the apparent power flow on line \( (i, j) \), and \( \overline{s}_{ij} \) is the corresponding limit.
\item ($\mathcal{E}$) denotes the set of power lines in the network.
\end{itemize}

%In equation (1), \( c_i(p_i) \) is a non-decreasing, upward-curving function, usually of a quadratic form or a stepwise linear representation, utilized to reflect the economics of adjustable active power generation accurately. 
 %The constraints in (3), (4), and (5) define the node voltage boundaries, node power injection limits, and line thermal capacities, respectively.

Our approach aims to predict with a graph neural network the pairs \( p \), \( q \)  for each generator that minimizes the objective function and enforces the domain constraints.





\begin{table}
  \centering
  \begin{tabular}{lll}
    Constraints formulae     & Penalty function   \\
    \hline
    $\omega_1 \land \omega_2$ & $\omega_1 + \omega_2$ \\
    $\omega_1 \lor \omega_2$ & $ \min(\omega_1, \omega_2)$ \\
    $\psi_1 \leq \psi_2$  & $max(0, \psi_1 - \psi_2)$   \\
    $\psi_1 < \psi_2$ & $max(0, \psi_1 - \psi_2 + \epsilon)$   \\
    
  \end{tabular}
  \caption{The grammar used to convert constraint formulae to penalty functions where $\epsilon$ is an infinitesimal value.}
  \label{tab:grammar-minimisation}
  \vspace{-1em}
 
\end{table}


The proposed OPF-HGNN framework is summarized in the Algorithm \ref{alg:opf-hgnn}. Lines 4-6 are for the mutation and simulation of our topologies, lines 7-14 are for the embedding generation, and lines 15-18 are for the loss computation used in backpropagation to update the weights of the model. 
\begin{algorithm}

  \caption{OPF-HGNN training of power grid $(\mathcal{N},\mathcal{E})$}
  \label{alg:opf-hgnn}
    \footnotesize
  \begin{algorithmic}[1]
  %-------------- Input & Output -----------------
  %\Require set of nodes of the power grid  $\mathcal{N}$ ; 
   \Require training graph $\mathbb{G}_t(\mathcal{N},\mathcal{E})$; 
   %\Require training input features $\{x_{t,v}, \forall v\in \mathcal{N}\}$; 
   %\Require constraints sets $\{\Omega_g, \forall g\in \mathcal{G}\}$;
   %\Require true active and reactive powers $\{\hat{y}_{t,g}, \forall g\in \mathcal{G}\}$;
   \Require  depth $K$; weight matrices $W^{k}, \forall k \in \{1,...,K\}$;
   %\Require non-linearity $\sigma$ / (ReLU for eg.);
    \Require aggregators $\textsc{aggregate}_k, \forall k \in \{1,...,K\}$;
    %\Require penalty to constraint mapping $\textsc{penalty}$;
    %\Require OPF simulation operator $\textsc{simulate}$;
    %\Require mutation operator $\textsc{mutate}$ ; 
    %\Require mutation rate $\mu$ and number of mutants $M$;
    \Require set of validation graphs $\mathcal{V}=\{\mathbb{G}_v(\mathcal{N},\mathcal{E})\}$;
    \Require neighborhood function $\mathcal{N} : v \rightarrow 2^{\mathcal{N}}$;
    %\Require neighbor sampling functions, $\mathcal{N}_k  \forall k \in \{1,...,K\}$;
      

  %--------------- for loop -----------------------
  
     
   \State $l \leftarrow 0$ \Comment{Initialize the epoch loss}

   \For{$m=1$ \textbf{to} M:}
        \Do
        \State $\mathbb{G}_v \leftarrow \textsc{mutate}$($\mathbb{G}_t$,$\mu$)
        \State valid$ , \{x_{m,v}\},\{\hat{y}_{m,g}\},\{\Omega_g\} \leftarrow \textsc{simulate}(\mathbb{G}_v)$ 
         \doWhile{$\mathbb{G}_v \in \mathcal{V}$ or $\neg$ valid}
          \State ${h}^0_v \leftarrow {x}_{m,v}, \forall v \in \mathcal{N}$ \;
         \For{$k=1...K$:}
         
              \For{$v \in \mathcal{N}$:}
            
               \State${h}^{k}_{\mathcal{N}(v)} \leftarrow \textsc{aggregate}_k(\{{h}_u^{k-1}, \forall u \in \mathcal{N}(v)\})$
                 \State    ${h}^k_v \leftarrow \textsc{ReLu} \left({W}^{k}\cdot\textsc{concat}({h}_v^{k-1}, {h}^{k}_{\mathcal{N}(v)})\right)$
               \EndFor
              \State ${h}^{k}_v\leftarrow {h}^{k}_v/ \|{h}^{k}_v\|_2, \forall v \in \mathcal{N}$
         \EndFor
         \State $\{y_{m,g}\} \leftarrow  \textsc{linear}(\{{h}^{K}_v,  \forall v \in \mathcal{N}\})$  \Comment{Regression}
         \State $l_{mse} \leftarrow \textsc{MSE}(\{y_{m,g}\},\{\hat{y}_{m,g}\})$
         \State $l_{penalty} \leftarrow \textsc{penalty}(\{y_{m,g}\},\{\Omega_g\})$ 
         \State $l \leftarrow l+ (l_{mse} + \lambda . l_{penalty})$ \Comment{Weighted penalty}
    \EndFor
    \State \Comment{Update weight matrices $W^{k}$ by backpropagation of $l$}

  %----------- Remaining text ----------------
  \end{algorithmic}
  
\end{algorithm}





==> pages/4.3-generalization.tex <==
% In this study, we evaluate the generalization capabilities of our approach with few-shot learning and transfer-learning. We summarize our results in Table \ref{tab:test_variation}.

% In the few-shot learning scenarios (scenarios (1), (2), and (3) in Table \ref{tab:test_variation}), we evaluate the cases where we only have a subset of the training grid (10\%) to train on, and evaluate how the performance of the model degrades compared to the full training scenario presented in Table \ref{tab:baseline_perf}.
% For load mutations, the results show no drop in constraint satisfaction between full training and few shot training and a marginal increase in MSE. These results hint that learning the impact of load changes does not require large training sets.
% There is, however, a significant drop in performances when predicting the OPF with varying generation costs and small training sets. Our results suggest that the impact of power generation costs on OPF optimization is significant and requires ten times more data to effectively learn how to enforce the constraints of the power grid. 

% Next, we investigate the transfer learning scenarios. We pre-train on the full training set of a source scenario, then fine-tune on 10\% of %the training set of 
% the target scenario. We summarize the results in scenarios (4-7). Our results show that the OPF-HGNN models completely transfer to smaller topologies, with low MSE and high constraint satisfaction. Meanwhile, training on small topologies can fail to generalize to larger topologies, especially with cost mutations. The bottleneck is constraint satisfaction, which seems harder to generalize to larger topologies.


% We compare in Table \ref{tab:baseline_perf} our approach and traditional GNN and FCNN when trained with the same features across three power systems. 
% The main takeway is that our approach OPF-HGNN achieves high constraint satisfaction across all the power systems, while the alternative approaches's constraint satisfaction collapses with increased size of power grids. For eg., OPF-HGNN achieves 98\% constraint satisfaction for 30-bus networks with mutated load powers. %This means that across the 2,000 validation graphs, for 40 graphs (2\%), the solution that OPF-HGNN predicted break the constraints of the power system.
% In addition to ensuring constraint satisfaction, our approach achives the lowest MSE in 20/24 scenarios and is up to three order of magnitude more precise than the alternatives. The MSE$_P$ of the active power for graphs with loads mutations is as low as about $1e^{-5}$ for our approach on the 9-bus case.% and around $1e^{-3}$ on the 30-bus case.
% \begin{figure*}
%     % \begin{subfigure}[b]{0.49\textwidth}
%     % \centering
%     % \includegraphics[width=\textwidth,trim=0 20px 0 20px, clip]{figures/ext_grid/case9_cost.png}
%     % \caption{WSCC 9-Bus w/ Cost mutations}
%     % \end{subfigure}
%     \begin{subfigure}[b]{0.49\textwidth}
%     \centering
%     \includegraphics[width=\textwidth,trim=0 20px 0 20px, clip]{figures/ext_grid/case9_load.png}
%     \caption{WSCC 9-Bus w/ Load mutations}
%     \end{subfigure}
%     % \begin{subfigure}[b]{0.49\textwidth}
%     % \centering
%     % \includegraphics[width=\textwidth,trim=0 20px 0 20px, clip]{figures/ext_grid/case14_cost.png}
%     % \caption{IEEE 14-Bus w/ Cost mutations}
%     % \end{subfigure}
%     \begin{subfigure}[b]{0.49\textwidth}
%     \centering
%     \includegraphics[width=\textwidth,trim=0 20px 0 20px, clip]{figures/ext_grid/case14_load.png}
%     \caption{IEEE 14-Bus w/ Load mutations}
%     \end{subfigure}

%     \caption{Predicted P of the external grid across 200 validation graphs on two topologies WSCC 9-Bus and IEEE 14-Bus with load mutations and few-shot learning. In blue the predicted values of our model and in orange the ground truth from the simulation.}
%     \label{fig:cases_mutations}
% \end{figure*}


% \begin{table*}[h!]
%   \centering
%   \caption{[OLD] Mean and Standard deviation of relative MSE in few-shot and transfer learning scenarios.}
  
%   \begin{tabular}{l|l|l|l|ll|ll|l}
%     ID & Cases & Training & Evaluation & \multicolumn{2}{c|}{MSE$_P$ MEAN\tiny{(STD)}}    & \multicolumn{2}{c|}{MSE$_Q$ MEAN\tiny{(STD)}}   & $CTR$ \\
%     & & & & External Grid & Generators  & External Grid  & Generators & \\
%     \toprule
%    (1) & 9-Bus $\rightarrow$ 9-Bus  & Load&Load & $2.15e^{-6}$\tiny{($3.40e^{-6}$)}& $9.77e^{-4}$\tiny{($1.51e^{-3}$)}&$7.85e^{-6}$\tiny{($1.24e^{-5}$)}&$5.08e^{-2}$\tiny{($1.68e^{-1}$)} & $1.00$\\
%    (2) & & Cost&Cost & $4.33e^{-3}$\tiny{($1.91e^{-2}$)} & $3.81e^{-3}$\tiny{($9.05e^{-3}$)}& $2.87e^{-3}$\tiny{($8.96e^{-3}$)}& $1.48e^{-1}$\tiny{($1.86$)}& $0.76$\\
%    (3) &  & Cost $\rightarrow$ Load&Load & $5.32e^{-4}$\tiny{($6.51e^{-4}$)}& $5.03e^{-4}$\tiny{($7.96e^{-4}$)}&$1.27e^{-2}$\tiny{($2.28e^{-2}$)}&$4.96e^{-3}$\tiny{($2.68e^{-2}$)} &$1.00$ \\
%    (4) &  & Load $\rightarrow$ Cost&Cost & $6.12e^{-2}$\tiny{($1.76e^{-1}$)}& $1.62e^{-2}$\tiny{($5.26e^{-2}$)}& $1.75e^{-3}$\tiny{($1.34e^{-1}$)}&$1.79e^{-2}$\tiny{($4.38e^{-1}$)} & $0.73$\\
%     \midrule
%    (5) & 14-Bus $\rightarrow$ 14-Bus & Cost&Cost & $1.30e^{-2}$\tiny{($3.59e^{-2}$)}& $5.10e^{-2}$\tiny{($1.01e^{-1}$)}&$4.58e^{-2}$\tiny{($8.73e^{-2}$)} &$1.13e^{-3}$\tiny{($1.16e^{-2}$)} &$0.52$\\
%    (6) &  & Load & Load & $4.98e^{-4}$\tiny{($5.78e^{-4}$)}& $2.48e^{-2}$\tiny{($2.52e^{-1}$)}&$3.57e^{-2}$\tiny{($2.44e^{-2}$)}&$1.07e^{-2}$\tiny{($1.88e^{-2}$)}&$0.84$\\
%    (7) & & Load $\rightarrow$ Cost&Cost & $3.19e^{-2}$\tiny{($7.25e^{-2}$)}& $9.94e^{-2}$\tiny{($2.76e^{-1}$)}& $2.36e^{-2}$\tiny{($6.67e^{-2}$)}&$1.34e^{-1}$\tiny{($1.81$)} & $0.22$\\
%    (8) & & Cost $\rightarrow$ Load&Load & $1.84e^{-6}$\tiny{($3.14e^{-6}$)}& $5.44e^{-2}$\tiny{($1.07e^{-1}$)}& $1.89e^{-2}$\tiny{($1.02e^{-3}$)}&$2.83e^{-3}$\tiny{($5.63e^{-3}$)} & $0.86$\\
%     \midrule
%    (9) & 9-Bus $\rightarrow$ 14-Bus& Cost&Cost & \tiny{()}& \tiny{()}& \tiny{()}&\tiny{()} & \\
%    (10) & & Load&Load & \tiny{()}& \tiny{()}& \tiny{()}&\tiny{()} & \\
%    (11) & 14-Bus $\rightarrow$ 9-Bus& Cost&Cost & \tiny{()}& \tiny{()}& \tiny{()}&\tiny{()} & \\
%    (12) & & Load&Load & \tiny{()}& \tiny{()}& \tiny{()}&\tiny{()} & \\
    
%   \end{tabular}
%   \label{tab:test_variation_old}
 
% \end{table*}


% \begin{table*}[h!]
%   \centering
%   \caption{Mean and Standard deviation of relative SE in few-shot and transfer learning scenarios.}
  
%   \begin{tabular}{l|l|l|ll|ll|l}
%     ID & Cases & Mutation & \multicolumn{2}{c|}{SE$_P$ MEAN\tiny{(STD)}}    & \multicolumn{2}{c|}{SE$_Q$ MEAN\tiny{(STD)}}   & $CTR$ \\
%     & & & External Grid & Generators  & External Grid  & Generators & satisfaction\\
%     \toprule
%    (1) & 9-Bus $\rightarrow$ 9-Bus  & Load & $2.15e^{-6}$\tiny{($3.40e^{-6}$)}& $9.77e^{-4}$\tiny{($1.51e^{-3}$)}&$7.85e^{-6}$\tiny{($1.24e^{-5}$)}&$5.08e^{-2}$\tiny{($1.68e^{-1}$)} & $1.00$\\
%    & & Cost & $4.33e^{-3}$\tiny{($1.91e^{-2}$)} & $3.81e^{-3}$\tiny{($9.05e^{-3}$)}& $2.87e^{-3}$\tiny{($8.96e^{-3}$)}& $1.48e^{-1}$\tiny{($1.86$)}& $0.76$\\
%    (2) &  14-Bus $\rightarrow$ 14-Bus& Load & $4.98e^{-4}$\tiny{($5.78e^{-4}$)}& $2.48e^{-2}$\tiny{($2.52e^{-1}$)}&$3.57e^{-2}$\tiny{($2.44e^{-2}$)}&$1.07e^{-2}$\tiny{($1.88e^{-2}$)}&$0.84$\\
%     &  & Cost & $1.30e^{-2}$\tiny{($3.59e^{-2}$)}& $5.10e^{-2}$\tiny{($1.01e^{-1}$)}&$4.58e^{-2}$\tiny{($8.73e^{-2}$)} &$1.13e^{-3}$\tiny{($1.16e^{-2}$)} &$0.52$\\
%    (3) &  30-Bus $\rightarrow$ 30-Bus& Load & $6.46e^{-5}$\tiny{($2.54e^{-4}$)}& $7.86e^{-4}$\tiny{($1.86e^{-3}$)}&$2.13e^{-1}$\tiny{($4.35e^{-4}$)}&$6.47e^{-4}$\tiny{($5.23e^{-3}$)}&$0.96$\\
%     &  & Cost & $1.53e^{-2}$\tiny{($2.90e^{-2}$)}& $1.31e^{-2}$\tiny{($4.14e^{-2}$)}&$7.74e^{-4}$\tiny{($6.32e^{-3}$)}&$4.59e^{-4}$\tiny{($8.25e^{-3}$)}&$0.73$\\
%     \midrule
%    (4) & 9-Bus $\rightarrow$ 14-Bus& Load &  7.44$e^{-6}$\tiny{($1.12e^{-5}$)}& $3.50e^{-1}$\tiny{($1.60$)}&$7.46e^{-3}$\tiny{($4.18e^{-3}$)}&$2.50e^{-2}$\tiny{($3.73e^{-2}$)}&$0.00$\\
%     & & Cost & $1.80e^{-2}$\tiny{($6.20e^{-2}$)}& $4.95e^{-2}$\tiny{($5.87e^{-1}$)}&$4.36e^{-2}$\tiny{($1.11e^{-1}$)}&$7.08e^{-1}$\tiny{($6.78$)} & $0.17$\\
%    (5) & 9-Bus $\rightarrow$ 30-Bus& Load &  $1.42e^{-4}$\tiny{($2.98e^{-3}$)}& $1.35e^{-2}$\tiny{($3.44e^{-2}$)}&$3.39e^{-5}$\tiny{($2.78e^{-4}$)}&$4.39e^{-3}$\tiny{($1.74e^{-2}$)}&$0.98$\\
%     & & Cost & $3.96e^{-2}$\tiny{($1.67e^{-1}$)}& $4.04e^{-2}$\tiny{($1.16e^{-1}$)}&$2.72e^{-3}$\tiny{($7.32e^{-3}$)}&$1.02e^{-3}$\tiny{($9.00e^{-2}$)}&$0.35$\\
%    (6) & 14-Bus $\rightarrow$ 9-Bus& Load & $1.61e^{-1}$\tiny{($2.01e^{-1}$)}& $3.87e^{-3}$\tiny{($4.76e^{-3}$)}&$2.86e^{-2}$\tiny{($8.10e^{-2}$)}&$8.76e^{-2}$\tiny{($3.20e^{-1}$)}&$1.00$\\
%     & & Cost & $1.42e^{-3}$\tiny{($3.41e^{-3}$)}& $3.61e^{-2}$\tiny{($8.43e^{-2}$)}&$6.44e^{-4}$\tiny{($1.04e^{-2}$)}&$2.71e^{-2}$\tiny{($1.50$)}& $0.75$\\
%    (7) & 30-Bus $\rightarrow$ 9-Bus& Load & $3.16e^{-5}$\tiny{($1.57e^{-4}$)}& $1.22e^{-4}$\tiny{($1.75e^{-4}$)}&$6.09e^{-3}$\tiny{($1.11e^{-2}$)}&$3.36e^{-4}$\tiny{($7.07e^{-2}$)}&$1.00$\\
%     & & Cost & $2.82e^{-4}$\tiny{($6.90e^{-4}$)}& $7.47e^{-3}$\tiny{($2.37e^{-2}$)}&$1.88e^{-3}$\tiny{($9.74e^{-3}$)}&$7.55e^{-3}$\tiny{($3.35e^{-2}$)}&$0.84$\\
%     \bottomrule
%   \end{tabular}
%   \label{tab:test_variation}
%   \vspace{-1em}
 
% \end{table*}


%\textbf{Few shot learning.}
%In this scenario...

%\textbf{Transfer learning}
%In this

==> pages/4.4-scalability.tex <==
% \begin{table}[]
% \centering
%   \caption{Graph NN model size (trainable weights) and inference time for 100.000 grids on CPU}
% \begin{tabular}{l|l|l|l|l}
% Case   &  \multicolumn{2}{c|}{HGNN} & \multicolumn{2}{c}{GNN} \\
%    &   Size & Time (sec) & Size  & Time (sec) \\
% \toprule
% Case9  &  555,052      & 458.46   & 27,076       & 67.53    \\
%        \midrule
% Case14    & 555,052      & 560.88  & 27,076       & 63.18    \\
%        \midrule
% Case30   & 555,052      & 607.61  & 27,076       & 71.44    \\
% \bottomrule
% \end{tabular}
% \label{tab:scalability_comparison}
% \end{table}

We compare in Table \ref{tab:scalability} how our models and inference time scale with the size of the system. Our results demonstrate that HGNN complexity is fixed whatever the size of the grid. The inference time scales linearly with the size of the grid. OPF-HGNN requires 4.58ms on one 9-Bus topology and 6.08ms on one 30-Bus topology. 
HGNN relies on message passing which generalizes with little overhead to large topologies\cite{liao_review_2022}.

\begin{table}[]
\centering
  \caption{Graph NN model size (trainable weights) and inference time for 100.000 grids on CPU}
\begin{tabular}{l|l|l|l|l|l}
  \multicolumn{2}{c|}{Case9} & \multicolumn{2}{c}{Case14} & \multicolumn{2}{c}{Case30} \\
 Size & Time (sec) & Size  & Time (sec) & Size  & Time (sec) \\
\toprule
 555,052      & 458.46   &555,052      & 560.88  & 555,052      & 607.61   \\

\bottomrule
\end{tabular}
\label{tab:scalability}
\vspace{-1em}
\end{table}
